On Coding for Cooperative Data Exchange

We consider the problem of data exchange by a group of closely-located wireless nodes. In this problem each node holds a set of packets and needs to obtain all the packets held by other nodes. Each of the nodes can broadcast the packets in its possession (or a combination thereof) via a noiseless broadcast channel of capacity one packet per channel use. The goal is to minimize the total number of transmissions needed to satisfy the demands of all the nodes, assuming that they can cooperate with each other and are fully aware of the packet sets available to other nodes. This problem arises in several practical settings, such as peer-to-peer systems and wireless data broadcast. In this paper, we establish upper and lower bounds on the optimal number of transmissions and present an efficient algorithm with provable performance guarantees. The effectiveness of our algorithms is established through numerical simulations.

==> ITW2010-random.tex <==

\section{Random Algorithms}\label{sec:random}

ALGORITHM-2 presented in the previous section requires some computation at every client at each iteration to determine the next best transmitting client. In some situations, it may be required to exchange packets in an ad-hoc and randomized manner.

      Let $c_1$ be an arbitrarily chosen first client. It only needs to transmit packets that are needed by at least one other client, which requires $\tau_1 = \max_{j\neq 1}\{|X_1 \cap \overline{X}_j|\}$ transmissions. The next randomly chosen client $c_2$ only needs to send $\tau_2 = \max_{j\neq 2}\{|X_2 \cap (\overline{X}_j \setminus X_1)|\}$ transmissions. And finally, $c_k$ only sends $\tau_k = \max_{j\neq k}\{|X_k \cap (\overline{X}_j \setminus (X_1 \cup X_1 \cup X_2 \cup \cdots \cup X_{k-1}))|\}$ transmissions. Therefore, for any given client ordering $\pi_r$, the number of transmissions is given by
\begin{align}\label{eq:Random}
    \tau_{\pi_r}= \sum_{j=1}^{k} \max_{i \neq j}\{|X_j \cap (\overline{X}_i \setminus (X_1 \cup \cdots \cup X_{j-1}))|\}.
\end{align}

The average number of transmissions in the random setting is simply the average taken over all possible $\pi_r$

\begin{align}\label{eq:Random:Ave}
    \overline{\tau} = \frac{1}{k!}\sum_{\pi_r}\tau_{\pi_r}.
\end{align}

